Differential Privacy in Aggregated Mobility Networks: Balancing Privacy and Utility

Location data is collected from users continuously to understand their mobility patterns. Releasing the user trajectories may compromise user privacy. Therefore, the general practice is to release aggregated location datasets. However, private information may still be inferred from an aggregated version of location trajectories. Differential privacy (DP) protects the query output against inference attacks regardless of background knowledge. This paper presents a differential privacy-based privacy model that protects the user's origins and destinations from being inferred from aggregated mobility datasets. This is achieved by injecting Planar Laplace noise to the user origin and destination GPS points. The noisy GPS points are then transformed into a link representation using a link-matching algorithm. Finally, the link trajectories form an aggregated mobility network. The injected noise level is selected using the Sparse Vector Mechanism. This DP selection mechanism considers the link density of the location and the functional category of the localized links. Compared to the different baseline models, including a k-anonymity method, our differential privacy-based aggregation model offers query responses that are close to the raw data in terms of aggregate statistics at both the network and trajectory-levels with maximum 9% deviation from the baseline in terms of network length.

==> savethis.tex <==
%\textit{degree of data transformation using noise injection for releasing geospatial statistics}

%\textit{degree of temporal aggregation is investigated to identify appropriate data releasing interval}

%\textit{business model privacy with fleet trajectories. Separate fleets and consumer datasets for experiments.}



%What the mathematical framework behind differential privacy enables is certainty about how much information about individuals “leaks” into calculations that are disclosed: how big must the random distortion to the average be in order to keep such leaks to an acceptable level? Specifying this level is what is called choosing “epsilon,” the Greek letter that is usually used as a measure of an upper bound of how much privacy may be lost.

 %We now have theoretical understandings of some of the fundamental limits on the number of queries that can be answered on a data set while preserving privacy, and at what level of accuracy. Hence, there will necessarily be tensions among researchers who will all want to use the same data for different purposes. How should these be resolved? Who gets to allocate priorities among researchers from different disciplines and methodological traditions? In the past, databases were seen as an evergreen resource — one person asking a question did not then limit another person’s ability to ask something. This is a fundamental shift in how data are viewed and will require significant structural changes in data governance.
 

%Transportation problems consist of two main concepts: demand, which tells the requests of populations in traffic, and supply, which provides the level of service of infrastructure. The general idea of solving the transportation problem is adjusting the service with respect to the demand. 



%The aggregation and disaggregation of transportation datasets has been studied for a very long time, mostly without considering privacy issues \cite{raadsen2020aggregation, steijn2016aggregation}. %???? what does this paper say?

% @mastersthesis{steijn2016aggregation,
%   title={Aggregation in Transport Networks for A Flexible Assignment Model},
%   author={Steijn, Justin},
%   year={2016},
%   school={University of Twente},
%   annote={This is a master thesis that studies aggregated zoning with several approaches. Basically they are proposing adaptive zoning based on the route availability between the zone centroids. Since they method is related to zone reconstruction, they only used road network model for a city without using a real dataset. Therefore, the problem is not related to privacy. }
% }


% @article{raadsen2020aggregation,
%   title={Aggregation, Disaggregation and Decomposition Methods in Traffic Assignment: Historical Perspectives and New Trends},
%   author={Raadsen, Mark PH and Bliemer, Michiel CJ and Bell, Michael GH},
%   journal={Transportation Research Part B: Methodological},
%   volume={139},
%   pages={199--223},
%   year={2020},
%   publisher={Elsevier},
%   annote={The paper reviews the aggergation and disaggreation methods for traffic assignment problem. For aggregation, they discussed the zone aggregation and network aggregation models for traffic assignment problems. }
% }





%It is still an open research question of how much information is lost with the developed differential privacy method because the quantification of information loss differs for different transportation problems. 
% Here we listed two example 

The proposed DP-ANI model does not classify locations to pre-defined groups, but rather matches them with the nearest links in offline mode. 


% @mastersthesis{steijn2016aggregation,
%   title={Aggregation in Transport Networks for A Flexible Assignment Model},
%   author={Steijn, Justin},
%   year={2016},
%   school={University of Twente},
%   annote={This is a master thesis that studies aggregated zoning with several approaches. Basically they are proposing adaptive zoning based on the route availability between the zone centroids. Since they method is related to zone reconstruction, they only used road network model for a city without using a real dataset. Therefore, the problem is not related to privacy. }
% }


% @article{raadsen2020aggregation,
%   title={Aggregation, Disaggregation and Decomposition Methods in Traffic Assignment: Historical Perspectives and New Trends},
%   author={Raadsen, Mark PH and Bliemer, Michiel CJ and Bell, Michael GH},
%   journal={Transportation Research Part B: Methodological},
%   volume={139},
%   pages={199--223},
%   year={2020},
%   publisher={Elsevier},
%   annote={The paper reviews the aggergation and disaggreation methods for traffic assignment problem. For aggregation, they discussed the zone aggregation and network aggregation models for traffic assignment problems. }
% }
